The Best Defense is Attack: Repairing Semantics in Textual Adversarial Examples

Recent studies have revealed the vulnerability of pre-trained language models to adversarial attacks. Existing adversarial defense techniques attempt to reconstruct adversarial examples within feature or text spaces. However, these methods struggle to effectively repair the semantics in adversarial examples, resulting in unsatisfactory performance and limiting their practical utility. To repair the semantics in adversarial examples, we introduce a novel approach named Reactive Perturbation Defocusing (Rapid). Rapid employs an adversarial detector to identify fake labels of adversarial examples and leverage adversarial attackers to repair the semantics in adversarial examples. Our extensive experimental results conducted on four public datasets, convincingly demonstrate the effectiveness of Rapid in various adversarial attack scenarios. To address the problem of defense performance validation in previous works, we provide a demonstration of adversarial detection and repair based on our work, which can be easily evaluated at https://tinyurl.com/22ercuf8.

==> motivation.tex <==
\section{Motivation}

\label{sec:arpd}
Our experiments show that reactive adversarial defense can almost avoid the clean performance sacrifice (refer to the experimental results in \pref{tab:clean}). Therefore, we propose a joint model for standard classification and adversarial detection and train this model based on multi-objective learning (a.k.a., multi-task learning). Moreover, we propose perturbation defocusing for adversarial defense and show its feasibility in \pref{tab:preliminary}. However, we cannot apply the perturbation mask in practical adversarial defense as we have no information about malicious perturbations. As a result, we propose adversarial attack-based perturbation defocusing, i.e., using adversarial attacks to generate enough safe perturbations. More specifically, we can obtain the adversarial detection results and standard classification outputs. While the adversarial detector identifies an adversary, the standard classification output is considered to be fake. Next, we feed the perturbed text and fake standard classification output into any adversarial attacker to search for perturbations (i.e., attack) which change the fake standard classification output. Because all perturbations (including malicious and safe perturbations) are generally designed to contain similar semantics (e.g., synonym substitutions), the objective models can correctly classify a text with a very high probability (our experiments indicate that the probability is over $97\%$.).

There are two advantages of using the adversarial attack-based for perturbation defocusing.

\begin{enumerate}[noitemsep,nolistsep,leftmargin=*]
	\item The search process for safe perturbations is supervised by the fake standard classification output. On the contrary, text or feature space reconstruction is not supervised. i.e., there is few information to guide reconstruction.
	\item Adversarial attack methods have great power to find enough perturbations to defocus malicious perturbations\footnote{The multiple adversarial attack methods-based perturbation defocusing can probably improve \our.}, which means that almost all adversarial samples can be repaired.
\end{enumerate}
